OSCAR: Data-Driven Operational Space Control for Adaptive and Robust Robot Manipulation

Learning performant robot manipulation policies can be challenging due to high-dimensional continuous actions and complex physics-based dynamics. This can be alleviated through intelligent choice of action space. Operational Space Control (OSC) has been used as an effective task-space controller for manipulation. Nonetheless, its strength depends on the underlying modeling fidelity, and is prone to failure when there are modeling errors. In this work, we propose OSC for Adaptation and Robustness (OSCAR), a data-driven variant of OSC that compensates for modeling errors by inferring relevant dynamics parameters from online trajectories. OSCAR decomposes dynamics learning into task-agnostic and task-specific phases, decoupling the dynamics dependencies of the robot and the extrinsics due to its environment. This structure enables robust zero-shot performance under out-of-distribution and rapid adaptation to significant domain shifts through additional finetuning. We evaluate our method on a variety of simulated manipulation problems, and find substantial improvements over an array of controller baselines. For more results and information, please visit https://cremebrule.github.io/oscar-web/.

==> tab-task_params.tex <==
\begin{table}
%   \setlength{\tabcolsep}{5pt} % Default value: 6pt - use this to pack table columns closer
  \begin{tabular}{ccccc}
    \toprule
    Task & Parameter & 
    \begin{tabular}[c]{@{}}Train\end{tabular} & \begin{tabular}[c]{@{}}Zero-Shot\end{tabular} & \begin{tabular}[c]{@{}}Adapt\end{tabular} \\
    \midrule
    \multirow{4}{*}{Common}
    & Joint Friction & $0.001 - 0.01$ & $0.01$ & $0.01$ \\
    & Joint Damping & $0.001 - 0.1$ & $0.1$ & $0.1$ \\
    & Joint Armature & $0.0002 - 0.005$ & $0.005$ & $0.005$ \\
    & Inertia Offset & $0.001 - 0.01$ & $0.01$ & $0.01$ \\
    \midrule
    \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Path\\Tracing\end{tabular}}
    & Path Shape & Circle & Square & "Robot" \\
    & Path Ori & Any & YZ-Plane & YZ-Plane \\
    & EEF Mass & $0.63 - 1.84$ & $3.18$ & $3.18$ \\
    \midrule
    \multirow{5}{*}{\begin{tabular}[c]{@{}c@{}}Cup\\Pouring\end{tabular}}
    & Num Particles & $10$ & $20$ & $100$ \\
    & Particle Density & $1000 - 20000$ & $20000$ & $20000$ \\
    & Particle Radius & $0.011$ & $0.011$ & $0.075$ \\
    & Cup Radius & $0.045 - 0.065$ & $0.05$ & $0.05$ \\
    & Cup Height & $0.1 - 0.2$ & $0.1$ & $0.15$ \\
    \midrule
    \multirow{8}{*}{\begin{tabular}[c]{@{}c@{}}Puck\\Pushing\end{tabular}}
    & Path Friction & $0.2 - 2.0$ & $4.0$ & $4.0$ \\
    & Path Incline & $0.0$ & $0.0$ & $0.1$ \\
    & Path Width & $0.09$ & $0.09$ & $0.08$ \\
    & Path Steps & $5$ & $5$ & $6$ \\
    & Puck Friction & $0.2 - 2.0$ & $2.5$ & $2.5$ \\
    & Puck Radius & $0.0325 - 0.0375$ & $0.0375$ & $0.0375$ \\
    & Puck Density & $1000 - 10000$ & $20000$ & $20000$ \\
    & EEF Mass & $0.1 - 2.0$ & $2.0$ & $2.0$ \\
    \bottomrule
  \end{tabular}
  \vspace{0.5em}
  \caption{\textbf{Task Parameters.} During normal task training, values are randomized uniformly between episodes. During zero-shot evaluation and adaptation finetuning, parameters are set to configurations unseen during training.}
  \label{tab:task_params}
% \vspace{-5pt}
\end{table}
